Inferring, Predicting, and Denoising Causal Wave Dynamics

The novel DISTributed Artificial neural Network Architecture (DISTANA) is a generative, recurrent graph convolution neural network. It implements a grid or mesh of locally parameterizable laterally connected network modules. DISTANA is specifically designed to identify the causality behind spatially distributed, non-linear dynamical processes. We show that DISTANA is very well-suited to denoise data streams, given that re-occurring patterns are observed, significantly outperforming alternative approaches, such as temporal convolution networks and ConvLSTMs, on a complex spatial wave propagation benchmark. It produces stable and accurate closed-loop predictions even over hundreds of time steps. Moreover, it is able to effectively filter noise -- an ability that can be improved further by applying denoising autoencoder principles or by actively tuning latent neural state activities retrospectively. Results confirm that DISTANA is ready to model real-world spatio-temporal dynamics such as brain imaging, supply networks, water flow, or soil and weather data patterns.

==> texts/relatedwork.tex <==
% Make the main file the master document for this file so that when compiling this file, actually the master file will be compiled. The name of the main file could also contain paths, like path/main.tex
% !TeX root = 2020-denoisingDISTANA.tex

\section{Related work}

As discussed in \cite{bai2018empirical}, sequences are traditionally modeled with recurrent neural networks.
However, recent findings increasingly suggest convolutional neural networks (CNNs)---and in particular temporal convolution netwoks (TCNs)---to model time series data \cite{kalchbrenner2016neural,dauphin2017language,bai2018empirical}.
ConvLSTM \cite{xingjian2015convolutional}, on the other hand, constitutes a convolution-gating LSTM architecture, which has proven powerful in systematic video prediction, such as sequential satellite images of clouds.

A particular way of interpreting data, however, is to consider them as graphs \cite{shuman2013emerging}, which comes with challenges (being not directly processable by traditional CNNs) and potentials (facilitating processing of irregularly distributed data); and promising neural network architectures that can operate on graphs have been proposed in the past \cite{gori2005new,scarselli2008graph,li2015gated,battaglia2018relational}.
A key aspect of these so called graph neural networks (GNNs) is an exclusive treatment of the two distinct components that make up graphs: graph nodes (vertices) and node connections (edges), which makes them applicable to a wide range of problems, such as classifying molecular properties \cite{gilmer2017neural}, processing images, videos \cite{santoro2017simple,watters2017visual,hu2018relation,van2018relational,wang2018non} and 3D point clouds \cite{wang2019dynamic}, or even simulating physical systems \cite{chang2016compositional,battaglia2016interaction,raposo2017discovering,santoro2017simple,watters2017visual,kipf2018neural,sanchez2018graph,van2018relational,karlbauer2019distributed}.  % TODO: eventually change to ESANN citation
For a review that focuses on applying CNNs on graphs, see \cite{bronstein2017geometric}, while \cite{wu2019comprehensive} constitutes a general survey on GNNs, which introduces four classes of GNNs, namely convolutional GNNs, graph autoencoders and spatial-temporal GNNs---we use the term spatio-temoral. Our model, DISTANA, belongs to the class of spatio-temporal GNNs (STGNNs) and shares architectural principles with \cite{jain2016structural}.

